Point-Based Value Iteration and Approximately Optimal Dynamic Sensor Selection for Linear-Gaussian Processes

The problem of synthesizing an optimal sensor selection policy is pertinent to a variety of engineering applications ranging from event detection to autonomous navigation. We consider such a synthesis problem over an infinite time horizon with a discounted cost criterion. We formulate this problem in terms of a value iteration over the continuous space of covariance matrices. To obtain a computationally tractable solution, we subsequently formulate an approximate sensor selection problem, which is solvable through a point-based value iteration over a finite "mesh" of covariance matrices with a user-defined bounded trace. We provide theoretical guarantees bounding the suboptimality of the sensor selection policies synthesized through this method and provide numerical examples comparing them to known results.

==> sensor_selection.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.5in,
height=1.5in,
at={(0,0)},
tick label style={font=\LARGE},
scale only axis,
xmin=0,
xmax=50,
xlabel style={font=\color{white!15!black},font=\LARGE},
xlabel={Time step, t},
ymin=1,
ymax=4,
ylabel style={font=\color{white!15!black},font=\LARGE},
ylabel={Sensor},
axis background/.style={fill=white}
]
\addplot[const plot, color=mycolor1, forget plot, line width=1.25] table[row sep=crcr] {%
1	3\\
2	1\\
3	4\\
4	2\\
5	1\\
6	2\\
7	1\\
8	4\\
9	2\\
10	1\\
11	2\\
12	1\\
13	4\\
14	2\\
15	1\\
16	2\\
17	1\\
18	4\\
19	2\\
20	1\\
21	2\\
22	1\\
23	4\\
24	2\\
25	1\\
26	2\\
27	1\\
28	4\\
29	2\\
30	1\\
31	2\\
32	1\\
33	4\\
34	2\\
35	1\\
36	2\\
37	1\\
38	4\\
39	2\\
40	1\\
41	2\\
42	1\\
43	4\\
44	2\\
45	1\\
46	2\\
47	1\\
48	4\\
49	2\\
50	1\\
};
\end{axis}

\end{tikzpicture}%
